Learning Theory Can (Sometimes) Explain Generalisation in Graph Neural Networks

In recent years, several results in the supervised learning setting suggested that classical statistical learning-theoretic measures, such as VC dimension, do not adequately explain the performance of deep learning models which prompted a slew of work in the infinite-width and iteration regimes. However, there is little theoretical explanation for the success of neural networks beyond the supervised setting. In this paper we argue that, under some distributional assumptions, classical learning-theoretic measures can sufficiently explain generalization for graph neural networks in the transductive setting. In particular, we provide a rigorous analysis of the performance of neural networks in the context of transductive inference, specifically by analysing the generalisation properties of graph convolutional networks for the problem of node classification. While VC Dimension does result in trivial generalisation error bounds in this setting as well, we show that transductive Rademacher complexity can explain the generalisation properties of graph convolutional networks for stochastic block models. We further use the generalisation error bounds based on transductive Rademacher complexity to demonstrate the role of graph convolutions and network architectures in achieving smaller generalisation error and provide insights into when the graph structure can help in learning. The findings of this paper could re-new the interest in studying generalisation in neural networks in terms of learning-theoretic measures, albeit in specific problems.

==> packages.tex <==

\usepackage{longtable}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage[english]{babel}

\usepackage{multicol}

% Set the size of the Headlines (\sections)
\usepackage{sectsty}
\sectionfont{\fontsize{10}{15}\selectfont}
\subsectionfont{\fontsize{10}{15}\selectfont}
\subsubsectionfont{\fontsize{10}{15}\selectfont}
\chapterfont{\fontsize{13}{15}\selectfont}


\usepackage{tabularx}
\usepackage{todonotes}

\usepackage{amsmath}
%center equations
	\makeatletter
	\@fleqnfalse
	\@mathmargin\@centering
	\makeatother
%%%
%theorem
\usepackage{amsthm}

\numberwithin{equation}{section}


% for numbering throught the whole documen
%\usepackage{chngcntr}
%\counterwithout{equation}{chapter}

\usepackage{tikz}
\usetikzlibrary{patterns,arrows,calc,decorations.pathmorphing}
\usetikzlibrary{matrix,chains,positioning,decorations.pathreplacing,arrows}
\usetikzlibrary{positioning,calc}
\usetikzlibrary{arrows,backgrounds}
\usetikzlibrary{angles,quotes}

\usepgflibrary{shapes.multipart}


\usepackage{float}
\usepackage{subcaption}


%jusefy
\usepackage{ragged2e}


\usepackage{amssymb}
\usepackage{bm} 
\usepackage{graphicx} 
\usepackage{pdflscape} 
\usepackage[bottom]{footmisc}
\usepackage{booktabs,caption,fixltx2e}
\usepackage[flushleft]{threeparttable}
\usepackage{tabularx}
\usepackage[toc,page]{appendix}
\usepackage{color}
\usepackage{array} 
\usepackage{arydshln}

\newcolumntype{R}{>{\raggedleft\arraybackslash}X} 
%\usepackage[style=alphabetic,backend=bibtex]{biblatex}	%authoryear
%\usepackage[style=authoryear]{biblatex}
%\usepackage[style=authoryear,natbib=true]{biblatex}
\usepackage[style=alphabetic,backend=bibtex]{biblatex}


%% integral over sum
\usepackage{graphicx}
\DeclareMathOperator*{\SumInt}{%
	\mathchoice%
	{\ooalign{$\displaystyle\sum$\cr\hidewidth$\displaystyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.14\height}{\scalebox{.7}{$\textstyle\sum$}}\cr\hidewidth$\textstyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
}



\usepackage{listings}
\usepackage{dsfont}
\newcommand\deff{\stackrel{def}{=}}
\usepackage{listings}
\lstset{
	breaklines=true,
	tabsize=4,
	%literate={\ \ }{{\ }}1
	numbers=left,
  	%stepnumber=5,    
 	firstnumber=1,
  	numberfirstline=true,
  	xleftmargin=2em,
  	%frame=single,
  	%framexleftmargin=1.5em
}

%\usepackage[singlespace]{setspace}
%\usepackage[onehalfspacing]{setspace}
\usepackage{setspace}
% \setstretch{1.5}


\usepackage{geometry}
\geometry{a4paper, top=20mm, left=30mm, right=30mm, bottom=20mm}

\usepackage[draft = false]{hyperref}

\hypersetup{hyperfootnotes = fales,	citebordercolor = blue,	colorlinks   = true, 	hyperfigures = true,	urlcolor     = blue, 	linkcolor    = blue, 	citecolor   = blue }


\ExecuteBibliographyOptions{maxcitenames=1}

\DeclareFieldFormat{citehyperref}{%
	\DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
	\bibhyperref{#1}}

\DeclareFieldFormat{textcitehyperref}{%
	\DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
	\bibhyperref{%
		#1%
		\ifbool{cbx:parens}
		{\bibcloseparen\global\boolfalse{cbx:parens}}
		{}}}

\savebibmacro{cite}
\savebibmacro{textcite}

\renewbibmacro*{cite}{%
	\printtext[citehyperref]{%
		\restorebibmacro{cite}%
		\usebibmacro{cite}}}

\renewbibmacro*{textcite}{%
	\ifboolexpr{
		( not test {\iffieldundef{prenote}} and
		test {\ifnumequal{\value{citecount}}{1}} )
		or
		( not test {\iffieldundef{postnote}} and
		test {\ifnumequal{\value{citecount}}{\value{citetotal}}} )
	}
	{\DeclareFieldAlias{textcitehyperref}{noformat}}
	{}%
	\printtext[textcitehyperref]{%
		\restorebibmacro{textcite}%
		\usebibmacro{textcite}}}

\addto\extrasenglish{%
	\renewcommand{\chapterautorefname}{\S}
	\renewcommand{\sectionautorefname}{\S}%
	\renewcommand{\subsectionautorefname}{\S}%
	\renewcommand{\appendixautorefname}{\S}
}

%DOTS I TABLE OF COTENT.
\usepackage{tocloft}

%\renewcommand\cftchapdotsep{\cftdotsep}
%\renewcommand\cftchapleader{\cftdotfill{\cftchapdotsep}}
%\renewcommand{\cftseader}{\cftdotfill{\cftdotsep}}


% change size of table of content headline
\renewcommand{\cfttoctitlefont}{\large\bfseries}
%chage size of appendices heasline
\renewcommand{\appendixpagename}{\large Appendices}
\renewcommand\cftloftitlefont{\large\bfseries}

%space aftter "contets"
\setlength\cftaftertoctitleskip{40pt}
\setlength\cftafterloftitleskip{50pt}

\setlength{\cftfigindent}{0pt}  % remove indentation from figures in lof
\setlength{\cfttabindent}{0pt}  % remove indentation from tables in lot

%numbering for subsubsection
\setcounter{secnumdepth}{3}
% https://divisbyzero.com/2008/09/22/what-is-the-difference-between-a-theorem-a-lemma-and-a-corollary/
\newtheorem{axiom}{Axiom}[section]
\newtheorem{conjecture}{Conjecture}[section]


\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[theorem]
\newtheorem{lemma}{Lemma}[theorem]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

\newcommand{\definitionautorefname}{Definition}
\newcommand{\axiomautorefname}{Axiom}
\newcommand{\conjectureautorefname}{Conjecture}
\newcommand{\propositionautorefname}{Proposition}
\newcommand{\lemmaautorefname}{Lemma}
\newcommand{\corollaryautorefname}{Corollary}
\newcommand{\exampleautorefname}{Example}



%\begin{theorem}[Pythagorean theorem]
%\begin{proof}

\usepackage{textcomp}

\usepackage{enumitem}
\usepackage[most]{tcolorbox}
%frame around text
\tcbset{
	frame code={}
	center title,
	left=0pt,
	right=0pt,
	top=0pt,
	bottom=0pt,
	colback=gray!10,
	colframe=gray!10,
	%width=\dimexpr\textwidth\relax,
	width=\textwidth,
	enlarge left by=-0.50mm,
	boxsep=5pt,
	arc=0pt,outer arc=0pt,
}


\usepackage{pstricks}

\usepackage{yfonts}
\usepackage{eufrak}

\usepackage{lipsum}
\newenvironment{Figure}
{\par\medskip\noindent\minipage{\linewidth}}
{\endminipage\par\medskip}


\def\doubleunderline#1{\underline{\underline{#1}}}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

\usepackage{chngpage}
\usetikzlibrary{cd}


% table of contents in each chapter
\usepackage{minitoc}




%% no spacing before align
\setlength{\abovedisplayskip}{0pt}%
\setlength{\belowdisplayskip}{0pt}%
\setlength{\abovedisplayshortskip}{0pt}%
\setlength{\belowdisplayshortskip}{0pt}%
\setlength{\jot}{0pt}% Inter-equation spacing


%\usepackage{mathtools}
%\mathtoolsset{showonlyrefs=true}
%\usepackage{autonum}


\usepackage[nameinlink,capitalize]{cleveref}

%% Arsham
%HTML code:	#91D0BB
%RGB code:	R: 145 G: 208 B: 187
%HSV:	160° 30.29% 81.57%

%% Seaborn blue
%HTML-code:	#417E90
%RGB-code:	R: 65 G: 126 B: 144
%HSV:	193.67° 54.86% 56.47%


\definecolor{blue}{RGB}{65,126,144}


\newif\ifmynotes
\mynotestrue
%\mynotesfalse
\definecolor{notetext}{rgb}{0.7,0,0}
\def\note#1{\ifmynotes\textcolor{red}{#1}\else\fi}



\usepackage{algorithm,float}

\usepackage[noend]{algpseudocode}
\usepackage{xargs}    

\newcommand{\tog}[1]{\todo[inline, color=green!40]{#1}}
\newcommand{\tob}[1]{\todo[inline,color=blue!40]{#1}}
\newcommand{\toi}[1]{\todo[inline]{#1}}



\usepackage{blkarray}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{graphicx}
\newcommand{\rdots}{\hspace{.2ex}\raisebox{1ex}{\rotatebox{-12}{$\ddots$}}}

